Towards Generalist Foundation Model for Radiology by Leveraging Web-scale 2D&3D Medical Data

In this study, we aim to initiate the development of Radiology Foundation Model, termed as RadFM. We consider the construction of foundational models from three perspectives, namely, dataset construction, model design, and thorough evaluation. Our contribution can be concluded as follows: (i), we construct a large-scale Medical Multi-modal Dataset, MedMD, which consists of 16M 2D and 3D medical scans with high-quality text descriptions or reports across various data formats, modalities, and tasks, covering over 5000 distinct diseases. To the best of our knowledge, this is the first large-scale, high-quality, medical visual-language dataset, with both 2D and 3D scans; (ii), we propose an architecture that enables visually conditioned generative pre-training, i.e., allowing for integration of text input with 2D or 3D medical scans, and generate responses for diverse radiologic tasks. The model was initially pre-trained on MedMD and subsequently fine-tuned on the domain-specific dataset, which is a radiologic cleaned version of MedMD, containing 3M radiologic visual-language pairs, termed as RadMD; (iii), we propose a new evaluation benchmark, RadBench, that comprises five tasks, including modality recognition, disease diagnosis, visual question answering, report generation and rationale diagnosis, aiming to comprehensively assess the capability of foundation models in handling practical clinical problems. We conduct both automatic and human evaluation on RadBench, in both cases, RadFM outperforms existing multi-modal foundation models, that are publicaly accessible, including Openflamingo, MedFlamingo, MedVInT and GPT-4V. Additionally, we also adapt RadFM for different public benchmarks, surpassing existing SOTAs on diverse datasets. All codes, data, and model checkpoint will all be made publicly available to promote further research and development in the field.

==> content/New_banchmark_results.tex <==
\begin{table}[t]
\footnotesize
\centering
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{18pt}
\caption{Description of the RadBench. Note that, considering many datasets are collected or generated from PMC papers, we split them on the paper-level, \emph{i.e.}, if a paper is randomly split into any test set, the arbitrary cases related to it will be dismissed in the whole training set, including for the two pre-training datasets, PMC-Inline and PMC-OA. For Rad3D series, we split them according to the published date of the cases, with those before 2023 as training data and the others as test data.
}
\vspace{3pt}
\begin{tabular}{lllc}
\toprule
Dataset Name & Task Description & Modalities & Split \\ 
\midrule
Rad3D-Modality & Modality Recognition  & Image / Text & \xiaoman{Split by date} \\
\midrule
VinDr-Mammo~\cite{vindrmammo} & Disease diagnosis & Image & Official split\\  
VinDr-SpineXR~\cite{vindrspine} & Disease diagnosis & Image & Official split\\ 
VinDr-PCXR~\cite{vindrpcxr} & Disease diagnosis & Image & Official split\\  
CXR-Mix~\cite{Wu2023KDiagKD} & Disease diagnosis & Image  & Official split\\
RadChest-CT~\cite{draelos_rachel_lea_2020_6406114}& Disease diagnosis & Image  & Official split\\
\midrule
PMC-VQA~\cite{Zhang2023PMCVQAVI} & Medical visual question answering  & Image / Text & Official split \\  
PMC-CaseReport & Medical visual question answering & Image / Text & Random split \\
VQA-RAD~\cite{lau2018dataset} & Medical visual question answering  & Image / Text & Official split\\
SLAKE~\cite{liu2021slake} & Medical visual question answering  & Image / Text & Official split\\
Rad3D-VQA & Medical visual question answering  & Image / Text & \xiaoman{Split by date}\\
\midrule
MIMIC-CXR~\cite{johnson2019mimic} & Report generation & Image / Text & Random split\\
Rad3D-Caption &  Report generation  & Image / Text & \xiaoman{Split by date}\\
MPx-Single & Report generation  & Image / Text & Random split\\
MPx-Multi & Report generation  & Image / Text & Random split\\
\midrule
Rad3D-Rationale & Rationale diagnosis.  & Image / Text & \xiaoman{Split by date}\\
\bottomrule
\end{tabular}
\footnotetext{}
\label{eval_data}
\end{table}

